Multi-Agent Reinforcement Learning from Delayed Marketplace Feedback for Objective-Weight Adaptation in Three-Sided Dispatch

Dispatch in three-sided marketplaces provides a natural setting for reinforcement learning from world feedback: decisions are evaluated by delayed operational outcomes such as delivery speed, courier utilization, and merchant congestion. We present a deployed reinforcement learning system at DoorDash that adapts dispatch objective weights in a large-scale food-delivery marketplace using delayed signals. Rather than replacing the combinatorial assignment optimizer, a store-level policy learned from logged marketplace data selects a discrete multiplier that shifts the dispatch optimizer's tradeoff between delivery quality and batching efficiency. This interface enables offline policy learning under noisy, delayed, and coupled feedback while preserving production feasibility constraints and operational safeguards. We train a shared value function using centralized offline data and decentralized store-level execution, with Double Q-learning targets and a conservative regularizer to reduce out-of-distribution value overestimation. In a production switchback experiment, the offline-trained policy increases batching and reduces courier-side time costs without degrading customer-facing delivery quality. Results illustrate how world feedback from a live economic and logistics system can be used to safely adapt decision policies online.

==> sections/1_intro.tex <==
\section{Introduction}
Food-delivery dispatch is a sequential decision problem embedded in a three-sided marketplace. Each assignment decision affects not only the current order but also downstream merchant backlog, courier availability, batching opportunities, and customer delivery quality. The platform must therefore repeatedly balance competing objectives: batching more aggressively can improve courier efficiency and reduce cost, while prioritizing faster execution can reduce lateness and improve customer experience \citep{ulmer2021restaurant,agatz2023crowdsourced}. In many production systems, this tradeoff is governed by static heuristic weights that are tuned globally and updated manually. Although operationally simple, such parameters are brittle under local, time-varying marketplace conditions.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/rl-dispatch.png}
    \caption{
    End-to-end Reinforcement learning workflow for dispatch objective-weight adaptation.
    During the online assignment run, each run step computes entity-level state features. The RL policy outputs an action corresponding to an entity-specific objective parameter, which is consumed by the downstream assignment optimizer. Offline, run identifiers are joined with delayed marketplace outcomes to construct rewards and training tuples for policy learning. The trained policy is then deployed back into the online serving path. The workflow supports both one-time offline training and iterative retraining as new production data becomes available.
    }
    \label{fig:rl-dispatch}
\end{figure}

This limitation is especially acute in large-scale dispatch systems, where the assignment objective must jointly account for customer speed, lateness, cancellations, courier utilization, batching, and cost. A single time-invariant parameter cannot adapt well across stores experiencing different real-time conditions. During peak congestion, over-batching can increase lateness and degrade quality; during slack periods, under-batching leaves efficiency gains unrealized. Our goal is therefore not to replace the full combinatorial assignment solver with an end-to-end reinforcement learning (RL) system. Instead, we learn a high-leverage objective-weight RL decision layer that adjusts batching preferences in real time while preserving the existing optimizer.

Prior work has studied RL for order dispatching, courier assignment, and routing in online food-delivery and meal-delivery systems \citep{chen2024matching,jahanshahi2022deep,zou2021online}. However, most existing studies focus on direct order-courier assignment or routing, often in offline or simulated settings. In contrast, our work studies production objective-weight adaptation for batching preferences: an offline RL policy does not replace the combinatorial assignment solver, but instead learns to adjust an objective weight embedded in a live dispatch loop. This setting presents a distinct challenge: batching directly couples merchant congestion, courier utilization, and customer lateness, and the effect of a local decision may only be observed through delayed downstream outcomes. This makes the problem both practically important and technically challenging for offline RL.

We present a deployed RL decision layer for real-time objective-weight adaptation in a large-scale food-delivery dispatch platform as illustrated in Figure \ref{fig:rl-dispatch}. The key idea is to decompose dispatch decision-making into a tractable discrete-action problem. Every 20 seconds, each store-level agent observes local marketplace state, including order backlog, courier wait times, fulfillment load, and supply-demand conditions, and selects an objective-weight multiplier from a small action set. This multiplier steers the existing assignment optimizer toward either batching efficiency or delivery speed. Agents execute independently at serving time, while training is centralized across stores using delayed reward signals aligned with system-level efficiency and quality. The learned policy is deployed in production, serving hundreds of millions of daily inferences at a 20-second decision cadence.

Our contributions are threefold. First, we introduce a production RL policy for dispatch that learns to adapt an optimizer objective weight rather than solving the full combinatorial assignment problem directly. Second, we formulate objective-weight adaptation for batching preferences as a multi-agent, delayed-reward offline RL problem aligned with a three-sided marketplace objective. Third, we demonstrate real-world impact from deployment: online experiments show consistent efficiency gains, increased batching, preserved delivery quality, and substantial annualized cost savings at production scale.

==> sections/2_agent.tex <==
\section{Objective-Weight Adaptation Agent}

We deploy reinforcement learning as an objective-weight adaptation layer inside an existing food-delivery dispatch system. The end-to-end workflow is illustrated in Figure~\ref{fig:rl-dispatch}. Rather than replacing the combinatorial assignment optimizer, the RL policy adapts an entity-level objective parameter that changes the optimizer's relative preference for delivery speed versus batching efficiency. This keeps the action interface small, preserves existing optimization and operational safeguards, and allows the policy to improve dispatch behavior without directly selecting courier-order assignments.

During each online assignment run, the system executes a sequence of run steps. At each step, state-processing logic computes entity-level marketplace features, which are passed to the RL policy as state $s$. The policy outputs an action $a$, represented as an entity-specific objective-weight multiplier. This multiplier is converted into an entity parameter and passed to the downstream assignment optimizer, which solves the assignment problem using the adapted objective before the run continues.

Offline, each assignment run is logged with a run identifier that links online decisions to delayed marketplace outcomes. A data-processing pipeline maps realized metrics, such as batching efficiency, delivery quality, and cost-related outcomes, back to the corresponding run information. These outcomes are converted into rewards and joined with states and actions to construct training tuples $(s_t, a_t, r_t, s_{t+1})$. A shared offline RL policy is trained from this dataset and deployed back into the online serving path.

==> sections/2a_problem.tex <==
\subsection{Problem Formulation}

We formulate dispatch objective-weight adaptation as a decentralized multi-agent decision process with centralized offline training. Let $\mathcal{I}=\{1,\ldots,N\}$ denote the set of stores, where each store $i \in \mathcal{I}$ is treated as an agent. At each assignment cycle $t$, every 20 seconds in production, store $i$ observes a local marketplace state $s_t^i \in \mathcal{S}$ and selects an action $a_t^i \in \mathcal{A}$ that adapts the relative priority of delivery speed versus batching efficiency. The problem is defined by the tuple
\begin{equation}
    \mathcal{M} =
    \left(
    \mathcal{I}, \mathcal{S}, \mathcal{A}, \mathcal{T}, R, \gamma, \lambda_0
    \right),
\end{equation}
where $\mathcal{I}$ is the set of store-level agents, $\mathcal{S}$ is the local state space, $\mathcal{A}$ is the discrete objective-weight adaptation action space, $\mathcal{T}$ denotes the transition dynamics induced by the production dispatch system, $R$ is a delayed multi-objective reward function, $\gamma$ is the discount factor, and $\lambda_0$ is the baseline delivery-speed objective weight used by the assignment optimizer.

\paragraph{State.}
The state $s_t^i$ is computed online at the store level and refreshed every 20 seconds. It contains real-time signals that characterize local store conditions:
\begin{equation}
    s_t^i =
    \left[
    d_t^i,\,
    \mathrm{sup}_t^i,\,
    \mathrm{cwt}_t^i\
    \right].
\end{equation}

Here, $d_t^i$ is the number of outstanding deliveries at store $i$, capturing local backlog. A high value generally indicates store-level congestion. The feature $\mathrm{cwt}_t^i$ denotes the median courier wait time at the store, capturing pickup friction. The feature $\mathrm{sup}_t^i$ is a localized supply-pressure estimate that adjusts a regional supply-pressure signal using store-level effective courier supply.

We compute $\mathrm{sup}_t^i$ because regional supply-pressure features can hide important store-level variation. For example, two stores in the same region may share the same regional supply-pressure value, but one store may have fewer feasible couriers considered by the assignment optimizer. To capture this difference, we estimate effective store-level supply from recent assignment runs. For each recently published delivery, the system records the number of feasible courier candidates that reached the optimization stage. We aggregate these candidate counts over a recent time window to obtain a store-level median effective supply $\widetilde{S}_t^i$. Let $\mathrm{sup}_t^{g(i)}$ denote the regional supply-pressure feature for the geographical region $g(i)$ containing store $i$, and let $\widetilde{S}_t^{g(i)}$ denote the median effective supply across stores in that region. We define
\begin{equation}
    \mathrm{sup}_t^i
    =
    \mathrm{sup}_t^{g(i)}
    \cdot
    \frac{\widetilde{S}_t^i}{\widetilde{S}_t^{g(i)}}.
\end{equation}
This rescaling increases the supply-pressure estimate for stores with fewer feasible couriers than the regional median and decreases it for stores with more feasible couriers. Together, $d_t^i$, $\mathrm{cwt}_t^i$, and $\mathrm{sup}_t^i$ allow the policy to distinguish stores that may share similar regional conditions but differ in local backlog, pickup friction, and effective courier supply.

\paragraph{Action.}
The action is a discrete multiplier that adjusts the delivery-speed weight used by the downstream assignment optimizer:
\begin{equation}
    a_t^i \in \mathcal{A}
    =
    \{0.8, 0.9, 1.0, 1.1, 1.2\}.
\end{equation}
Lower values bias the optimizer toward batching efficiency, while higher values bias it toward faster delivery. The neutral action $a_t^i=1.0$ recovers the baseline behavior. The policy therefore does not select courier-order assignments directly; instead, it learns how to adapt an existing optimizer objective at the store level.

\paragraph{Reward.}
The reward is computed from delayed delivery outcomes and is aggregated at the regional level to capture network effects across nearby stores and couriers. Although each store acts as an independent agent at serving time, its action can affect courier availability, batching opportunities, and downstream assignment quality beyond that store. We therefore attribute rewards using outcomes from the surrounding dispatch region rather than only from the focal store.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/reward.png}
    \caption{xxxxx}
    \label{fig:rl-reward}
\end{figure*}

For each delivery $j$, let $t_j^{\mathrm{create}}$ denote the order creation time, $t_j^{\mathrm{acc}}$ denote the courier acceptance time, and $t_j^{\mathrm{drop}}$ denote the delivery dropoff time. We define realized delivery duration as
\begin{equation}
    \mathrm{ASAP}_j
    =
    t_j^{\mathrm{drop}} - t_j^{\mathrm{create}} .
\end{equation}
This term captures customer-facing delivery speed. We define delivery-level courier active time as
\begin{equation}
    \mathrm{CAT}_j
    =
    t_j^{\mathrm{drop}} - t_j^{\mathrm{acc}} .
\end{equation}
For a batched route, deliveries in the same batch may share the same acceptance time but have different dropoff times, so later dropoffs receive larger delivery-level active time. We then define delivery-level excess active time as
\begin{equation}
    \mathrm{XCAT}_j
    =
    \mathrm{CAT}_j
    -
    T_j^{\mathrm{direct}} .
\end{equation}
Here, $T_j^{\mathrm{direct}}$ represents the direct pickup-to-dropoff travel time for delivery $j$ if served alone, while $\mathrm{XCAT}_j$ captures the additional active-time burden induced by assignment, batching, waiting, and routing. Efficient batching yields small excess active time, whereas inefficient batching or poor routing increases $\mathrm{XCAT}_j$.

Let $\mathcal{D}_t^{g(i)}$ denote the set of deliveries in the dispatch region $g(i)$ associated with store $i$ whose delayed outcomes are attributed to decision cycle $t$. The reward is
\begin{equation}
    r_t^{g(i)}
    =
    -
    \frac{1}{|\mathcal{D}_t^{g(i)}|}
    \sum_{j \in \mathcal{D}_t^{g(i)}}
    \left(
        \alpha \, \mathrm{ASAP}_j
        +
        \beta \, \mathrm{XCAT}_j
    \right).
\end{equation}
The first term penalizes customer delivery duration, while the second penalizes excess courier active time beyond direct pickup-to-dropoff travel. Aggregating the reward at the regional level discourages store-level agents from optimizing  for local outcomes and better aligns learning with the marketplace-wide effects of batching decisions.

==> sections/2b_train.tex <==
\subsection{Offline Training}

Let $\pi_\theta(a \mid s)$ denote the shared store-level policy. Each store executes the policy independently using local state, while training pools experience across stores and uses regional rewards to capture cross-store network effects. This centralized-training, decentralized-execution design is important because a store-level action can affect courier availability, batching opportunities, and delivery quality beyond the focal store.

A transition pipeline joins each online decision with delayed fulfillment and delivery outcomes to construct an offline dataset
\begin{equation}
    \mathcal{D}
    =
    \{(s_t^i, a_t^i, r_t^{g(i)}, s_{t+1}^i)\},
\end{equation}
where each tuple corresponds to a store-level decision, $g(i)$ denotes the dispatch region containing store $i$, and $r_t^{g(i)}$ is the realized regional reward attributed to that decision cycle. Even with limited exploration exposure, the system produces millions of logged transitions per day, enabling rapid offline iteration. The goal is to learn a policy that maximizes expected discounted regional reward:
\begin{equation}
    \pi^*
    =
    \arg\max_{\pi_\theta}
    \mathbb{E}_{\pi_\theta}
    \left[
    \sum_{t=0}^{H}
    \gamma^t r_t^{g(i)}
    \right].
\end{equation}

\paragraph{Value learning.}
We train a discrete-action value function $Q_\theta(s,a)$ using a DQN-style offline objective \citep{mnih2015dqn}. For a transition $(s_t^i,a_t^i,r_t^{g(i)},s_{t+1}^i) \in \mathcal{D}$, standard DQN uses the temporal-difference target
\begin{equation}
    y_t
    =
    r_t^{g(i)}
    +
    \gamma
    \max_{a' \in \mathcal{A}}
    Q_{\bar{\theta}}(s_{t+1}^i, a'),
\end{equation}
where $Q_{\bar{\theta}}$ is a target network and $\gamma$ is the discount factor. In early iterations, this objective exhibited a common offline RL failure mode: actions weakly supported by the logged data could receive overestimated values, reducing policy reliability.

To reduce maximization bias, we use Double DQN targets \citep{vanhasselt2016double}. The online network selects the next action, while the target network evaluates it:
\begin{equation}
    a_t^*
    =
    \arg\max_{a' \in \mathcal{A}}
    Q_{\theta}(s_{t+1}^i, a'),
\end{equation}
\begin{equation}
    y_t^{\mathrm{DDQN}}
    =
    r_t^{g(i)}
    +
    \gamma
    Q_{\bar{\theta}}(s_{t+1}^i, a_t^*) .
\end{equation}
The resulting temporal-difference loss is
\begin{equation}
    \mathcal{L}_{\mathrm{DDQN}}(\theta)
    =
    \mathbb{E}_{(s,a,r,s') \sim \mathcal{D}}
    \left[
    \left(
    Q_\theta(s,a) - y^{\mathrm{DDQN}}
    \right)^2
    \right].
\end{equation}

\paragraph{Conservative regularization.}
Double DQN reduces maximization bias, but offline training still faces distribution shift between the logged behavior policy and the learned policy. To discourage unsupported actions from receiving high values, we add a discrete Conservative Q-Learning regularizer \citep{kumar2020cql}. For each logged state-action pair $(s,a) \sim \mathcal{D}$, we use
\begin{equation}
    \mathcal{L}_{\mathrm{CQL}}(\theta)
    =
    \mathbb{E}_{(s,a) \sim \mathcal{D}}
    \left[
    \log \sum_{a' \in \mathcal{A}}
    \exp Q_\theta(s,a')
    -
    Q_\theta(s,a)
    \right].
\end{equation}
This penalty increases the loss when actions other than the logged action receive high Q-values, encouraging conservative estimates for actions not well supported by the offline data.

The final objective is
\begin{equation}
    \mathcal{L}(\theta)
    =
    \mathcal{L}_{\mathrm{DDQN}}(\theta)
    +
    \eta
    \mathcal{L}_{\mathrm{CQL}}(\theta),
\end{equation}
where $\eta$ controls the strength of conservatism. In practice, this combination trades off faster convergence for more conservative value estimates and more stable deployment behavior.

==> sections/a_related_work.tex <==

\section{Related Work}

Prior work has studied RL for operational decision-making in meal-delivery systems, including order dispatching, courier assignment, routing, repositioning, and batching. \citet{chen2024matching} propose an RL-based matching method for real-time order-rider assignment in on-demand meal delivery. \citet{jahanshahi2022deep} formulate meal delivery as an MDP and apply deep RL to courier assignment, order rejection, and repositioning, while \citet{zou2021online} study online food-order delivery strategies with Double DQN in simulation. Other work considers related operational problems such as concurrent instant-delivery dispatch, adaptive buffering and dynamic batching, and joint dispatching with idle-fleet steering \citep{guo2021concurrent,lu2024abod,cheng2025realtime}. In contrast, our work does not learn direct order-courier matchings, routes, or batching decisions; instead, it learns an objective-weight adaptation policy that modulates an existing combinatorial assignment optimizer and is evaluated through online production experiments.

Industrial marketplace systems often introduce learning-based methods as constrained decision layers inside larger optimization pipelines. Early industry work explored RL for on-demand logistics by selecting among parameterized assignment variants in simulation \citep{hwang2018doordash}, while marketplace-balance work has used offline value functions to augment online matching systems \citep{bakhtiari2025uber}. Related marketplace layers have also adopted bandit methods for ranking and retrieval, with randomized data collection and off-policy evaluation \citep{wang2018ubereats,vengerov2023instacart}. These systems motivate a practical design pattern: learning-based policies are often safest when they operate over constrained interventions rather than replacing core production optimizers end to end.

Methodologically, our approach builds on centralized training with decentralized execution (CTDE) and offline value-based RL. CTDE enables centralized aggregation of experience while preserving local, low-latency serving decisions \citep{amato2024ctde}. Offline RL must address distribution shift between logged data and the learned policy; Conservative Q-Learning regularizes learned Q-values to reduce overestimation on unsupported actions \citep{kumar2020cql}. Double Q-learning and Double DQN reduce maximization bias by decoupling action selection from action evaluation \citep{vanhasselt2016double}. We combine these ideas in a discrete-action DQN-style offline learner for production objective-weight adaptation.
